AGSTN: Learning Attention-adjusted Graph Spatio-Temporal Networks for Short-term Urban Sensor Value Forecasting

Forecasting spatio-temporal correlated time series of sensor values is crucial in urban applications, such as air pollution alert, biking resource management, and intelligent transportation systems. While recent advances exploit graph neural networks (GNN) to better learn spatial and temporal dependencies between sensors, they cannot model time-evolving spatio-temporal correlation (STC) between sensors, and require pre-defined graphs, which are neither always available nor totally reliable, and target at only a specific type of sensor data at one time. Moreover, since the form of time-series fluctuation is varied across sensors, a model needs to learn fluctuation modulation. To tackle these issues, in this work, we propose a novel GNN-based model, Attention-adjusted Graph Spatio-Temporal Network (AGSTN). In AGSTN, multi-graph convolution with sequential learning is developed to learn time-evolving STC. Fluctuation modulation is realized by a proposed attention adjustment mechanism. Experiments on three sensor data, air quality, bike demand, and traffic flow, exhibit that AGSTN outperforms the state-of-the-art methods.

==> 2-RelatedWork.tex <==
\section{Related Work}
\label{sec-related}
\textbf{Urban Spatio-Temporal Forecasting.}
Since sensors are deployed in different geographical urban areas and evolved (e.g., monitoring stations of PM2.5 and traffic flow), existing studies have developed various spatio-temporal forecasting methods to model how the time series of sensors are correlated with each other. Autoregression-based models (e.g., ARIMA) are typical approaches to forecast sensor time series, but they cannot model the spatial correlation. Zheng et al.~\cite{zheng15} propose a multi-modal data fusion-based approach that effectively models temporal and spatial factors and generate air quality predictions. Liu et al.~\cite{uwater16} develop a multi-task multi-view learning method that fuses multiple datasets to model the spatio-temporal correlation regarding sensor time series. With the development of deep sequential learning~\cite{seq2seq}, a variety of studies have utilized short-term memory (LSTM), gated recurrent unit (GRU), and convolutional neural networks to jointly model the spatial and temporal dependency~\cite{cnn1,cnn2,rnn1,rnn2}. Attention-based models had shown promising performance in learning to select the useful features and encoder hidden vectors in different applications~\cite{att1,att2}. For geo-sensory time series prediction, a dual-stage attention-based recurrent neural network (DARNN)~\cite{darnn} to select the relevant driving series at each time interval. A multi-level attention network, GeoMAN~\cite{geoman}, can further improve the performance by modeling dynamic spatio-temporal dependencies and incorporating multiple sensors' readings with cross-domain datasets. 

\textbf{Graph-based Neural Network Models.}
Graph neural network-based (GNN) models~\cite{gnnsvy,GCNpaper} have been investigated and applied to different domains, and have promising performance recently. The power of GNNs lies in depicting the relationships between sensors by different graph structures, and learning the feature representation of each sensor node through their neighbors in the graphs. Hsieh et al.~\cite{unoise} construct multi-source spatio-temporal graphs, along with label propagation-based random walk, to predict urban noise. STG2Vec~\cite{stg2vec} learns the sensor representations from a heterogeneous spatial-temporal graph, constructed from dynamic bike transition networks, to predict bike-sharing demand.
DGCNN~\cite{dgcnn} utilizes road networks of road segments to build the dynamic graph convolutional neural network model for Traffic forecasting. ST-MGCN~\cite{stmgcn} leverages geographical nearest-neighbors, region functions, and transportation connectivity to create multiple graphs to model spatial correlation between sensors, and apply graph convolutional networks (GCN)~\cite{GCNpaper} for ride-hailing demand forecasting. ST-GCN~\cite{stgcn} and AST-GCN~\cite{astgcn} apply GCNs to existing road and traffic networks to capture the spatio-temporal patterns among sensors for traffic flow prediction. PM2.5-GNN~\cite{pm25gnn} constructs a knowledge graph from various datasets in the meteorology domain, and accordingly devises a GNN model for air quality forecasting.


\textbf{Short Summary.} 
Although these above-discussed models have reached some success, some rely on multi-source datasets to learn spatio-temporal correlation, and train the model separately for each senor. Some previous models fit only specific geo-sensory data (e.g., air quality PM2.5, traffic flow, urban noise, and bike demand), i.e., cannot be generalized to tackle diverse sensor data. For graph neural network-based approaches, most of the existing studies require the pre-defined graph structures so that the node/sensor embeddings can be learned and generated. Besides, none of them consider the variety of fluctuation (e.g., scale, frequency, and duration of fluctuation) of different sensors' time series. 
In this work, we aim at utilizing only time-series data, i.e., no multi-source datasets, to forecasting values of urban sensors. The proposed AGSTN model is not data-specific, and can be applied to different geo-sensory data. AGSTN also does not rely on pre-defined graphs, and is able to deal with various fluctuations of time series.


